Efficient Learning and Decoding of the Continuous-Time Hidden Markov Model for Disease Progression Modeling

The Continuous-Time Hidden Markov Model (CT-HMM) is an attractive approach to modeling disease progression due to its ability to describe noisy observations arriving irregularly in time. However, the lack of an efficient parameter learning algorithm for CT-HMM restricts its use to very small models or requires unrealistic constraints on the state transitions. In this paper, we present the first complete characterization of efficient EM-based learning methods for CT-HMM models, as well as the first solution to decoding the optimal state transition sequence and the corresponding state dwelling time. We show that EM-based learning consists of two challenges: the estimation of posterior state probabilities and the computation of end-state conditioned statistics. We solve the first challenge by reformulating the estimation problem as an equivalent discrete time-inhomogeneous hidden Markov model. The second challenge is addressed by adapting three distinct approaches from the continuous time Markov chain (CTMC) literature to the CT-HMM domain. Additionally, we further improve the efficiency of the most efficient method by a factor of the number of states. Then, for decoding, we incorporate a state-of-the-art method from the (CTMC) literature, and extend the end-state conditioned optimal state sequence decoding to the CT-HMM case with the computation of the expected state dwelling time. We demonstrate the use of CT-HMMs with more than 100 states to visualize and predict disease progression using a glaucoma dataset and an Alzheimer's disease dataset, and to decode and visualize the most probable state transition trajectory for individuals on the glaucoma dataset, which helps to identify progressing phenotypes in a comprehensive way. Finally, we apply the CT-HMM modeling and decoding strategy to investigate the progression of language acquisition and development.

==> CTHMM_decode/Chapter4_CTHMMdecoding.tex <==
\section{CTMC End-State Conditioned Optimal State Path Decoding and Computation of Expected State Duration}
%Path-Conditioned 

In this chapter, we will first review the prior work that tackles optimal state sequence decoding given two end-states and a total time. We will review two possible settings for the decoding problems. One is to find the most likely state and duration sequence \cite{Perkins2009NIPS}, and the other is to find the most probable state sequence considering all possible duration assignments \cite{Levin2012}. These decoding problems have practical use, such as ... \cite{Perkins2009NIPS}, and can be used in both CTMC and CT-HMM models. 

For the first problem setting which inferring the most likely state and duration sequence (a trajectory which is a sequence of states as well as the exact amount of time spent in each state), it is noted recently \cite{Perkins2009NIPS} that this problem appears unsolved before. \cite{Perkins2009NIPS} then solve this problem in three settings: (1) given the starting state and a total time; (2) given both the starting state and the end state, with the total time; (3) given a set of observed states in irregularly space times, with a total time. The task is to seek the most likely trajectory that passes through the given states at the specified times. The paper \cite{Perkins2009NIPS} shows that maximum likelihood trajectory is not always well-defined if the model has a specific property (explain more later), and this property can be checked using a polynomial time procedure. When well-definedness holds, the author provides exact and dynamic programming algorithm for inferring the most likely trajectories of CTMCs under the above mentioned three settings. It is found in \cite{Perkins2009NIPS} that the most likely dwell times are often infinitessimal and non-representative of typical system behavior.
%, while the problem is not always well-defined. 

The second problem setting is to find the most probable state sequence only while marginaling out the state dwell time. This setting has probability rather than likelihood, which always exist a best solution. This problem is recently solved in \cite{Levin2012}, which guarantee to find the best solution using a path extending and pruning algorithm. The possible downside of the algorithm in \cite{Levin2012} is that the time complexity depends in a complex way of the underlying state transition matrix $Q$ and the specified total time. There is currently no easy time complexity analysis of the method, but it is guaranteed to terminate in finite time.
%and in the worst case, an exhaustic searching may happen.

%%% CT-HMM case
%In terms of  CT-HMM, existing methods for CT-HMM decoding, generally refers to the decoding of the outer state sequence, where each decoded state corresponds to one actual observation. The outer state sequence decoding can be easily done by using \textit{Viterbi} algorithm, as it is conducted for DT-HMM, but a time-dependent transition probability matrix $P(t)$ is needed. As the outer state sequence decoding is solved by \textit{Viterbi} method,	in this chapter we focus on solving the problem that finds the optimal inner state chain given two known end-states and a total time.

%% why compute expected duration
In the second problem setting, \cite{Levin2012} finds the optimal state sequence considering all possible durations. \cite{Levin2012} computes the probability of a feasible state sequence given a total time $t$ by solving Kolmogorov-Chapman equations using numerical methods for ODE, and it can output the probability for a grid of time points from 0 to $t$, which are used in prunning the paths in the dynamic program algorithm. In this dissertation, we derive an efficient closed-form expression to compute the probability of a state sequence given a total time $t$ in $O(n^2)$ where $n$ is the path length, when the holding time parameters $q_i$ in the path are distinct. Our closed-form provides an efficient method to compute the same statistics which can also be used in inference tasks using sampled-paths  \cite{Hajiaghayi2014}.

In addition, in the second problem setting, it will also be useful to derive the expected state duration for each state in the optimal path. Both the state sequence and the expected state durations can be used in applications that require trajectory comparison and clustering. We derive the closed-form 
expression for efficiently computing these statistics when $q_i$ in the path are distinct, which has time complexity $O(n^2)$ for computing only one state, and $O(n^3)$ for all states in the path. Our closed-form solution doesn't require matrix multiplication, and is more efficient than applying other alternative methods (Expm, Unif, Eigen), which needs at least $O(n^3)$ for computing expectation for one state.

Our main contributions are summarized as follows:
\begin{itemize}
	\item We derive a closed-form formulation to evaluate the total time conditioned state sequence probability, which has time complexity of $O(n^2)$, where $n$ is the length of the state sequence. The direct method to compute this probability using matrix exponential requires $O(n^3)$ time.	
	\item We derive a closed-form formulation to compute the expected state duration for each state given a state path and a total time. Our closed-form has time complexity of $O(n^2)$ to compute for just one state, and $O(n^3)$ to compute for all states along the path. The competing methods require at least $O(n^3)$ for just one state, because these method all require matrix multiplication. 	
	%in the path-and-time conditioned optimal state sequence.
\end{itemize}

This chapter is organized as follows. In Section \ref{decode:prior_work}, we review the prior work for CTMC end-state and time conditioned optimal state sequence decoding. In Section \ref{sec:effi_statepath_prob}, we review the known closed-form formulation to compute the time-conditioned state sequence probability using matrix exponential, and then derive our new expression to compute the same statistics without using matrix multiplication which is more time efficient. In Section \ref{sec:effi_state_expect}, we derive our closed-form expression to compute the path and time-conditioned expected state duration. We will compare the time complexity of our new closed-form to alternative methods using \textit{Expm, Unif, Eigen} on an auxiliary transition matrix in computing the same statistics. 

% =================================================

\section{Prior work on CTMC state sequence decoding}

\label{decode:prior_work}

In Section \ref{sec:decode_state_path}, we will review the work for finding the most probable state sequence considering all possible duration assignments, as this setting always has a best solution, and can is useful in real applications \cite{Levin2012}. In Section \ref{sec:decode_max_like}, we will then review the work that finds the maximum likely state and duration sequence \cite{Perkins2009NIPS} and explain in what condition the maximum likely solution does not exist.

% ============================================

\subsection{Search for maximum probability state sequences considering all continuous duration assignments}

\label{sec:decode_state_path}

The setting in \cite{Levin2012} is to search the maximum probability state sequence considering all possible duration assignments bounded by two end-states and total duration $T$. The formulation is as follows. Given a CTMC = $(S, Q)$, where $S$ is the state set and $Q$ is the transition matrix. Define the time-dependent probability of a state sequence $P_t(G)$ as the probability that the chain visits precisely the sequence of states in $G = (s_1, ..., s_n)$ by time $t$ given that it starts at $s_1$ at time 0. Let $\tau_1, \tau_2, ..., \tau_n$ be dwell time in the states in $G$, define:
\begin{align}
P_t(G) = (\prod_{i=1}^n v_{s_i, s_{i+1}}) p(\sum_{i=1}^{n-1} \tau_i \leq t \leq \sum_{i=1}^n \tau_i).
\end{align}
The goal is to evaluate $P_t(G)$ over a time interval $[0 t]$, which needs in the path extending and prunning algorithm \cite{Levin2012}.

To evaluate $P_t(G)$, \cite{Levin2012} used the Chapman-Kolmogorov equations, resulting in:
\begin{align}
\frac{d P_t(G)}{dt} = q_{s_{n-1}} v_{s_{n-1}, s_n} P_t(\bar{G}) - q_{s_n} P_t(G)
\end{align}
where $\bar{G}$ is the state sequence $(s_1, ..., s_{n-1}$, that is, one-step shorter sequence of the states in $G$. To evaluate $P_t(G)$, one needs to solve the above linear differential equation. This equation depends on $P_t(\bar{G})$, which obeys its own linear differential equation, depending in part on the probability of a state sequence which is yet one step shorter. Thus, one can find $P_t(G)$ by solving system of linear differential equations, where the variables are $P_t((s_1))$, $P_t((s_1, s_2))$, ..., $P_t((s_1, s_2, ..., s_n))$. The initial conditions are $P_t((s_1))=1$ and $P_t((s_1,..., s_i))=0, i>0$. One can use standard numerical methods to solve differential equations to calculate $P_t(G)$.

Then, to find the optimal state sequence given a total time $t_{max}$, \cite{Levin2012} proposed a way to guide the path extending and prunning process using a notion called \textit{dominance}. Suppose $G_1$ and $G_2$ are two different state sequences with same starting and end state. Then $G_1$ dominates $G_2$ if $P_t(G_1) > P_t(G_2)$ for all $t \in (0, t_{max})$. If $G$ is not dominated by any other sequence, then $G$ is said non-dominated. \cite{Levin2012} proves that if the given CTMC has a finite state set, then there must be a finite number of non-dominated state sequences given a total time $t_{max}$. Then, if the program can list them all, and check which has the largest probability, then the maximum probability sequence is guaranteed to be found. \cite{Levin2012} also shows that all prefixes of any non-dominated sequence must also be non-dominated. 

\cite{Levin2012} proposes a search and prunning algorithm that enumerates non-dominated sequences from shorter to longer, starting from the specified starting states. After enumerating, each non-dominated sequence is evaluated to see which is the most probable one at time $t_{max}$. Please see \cite{Levin2012} for the detailed algorithm.

%\begin{figure}[htb]
%	\centering		
%	\includegraphics[width=0.50\linewidth]{CTHMM_decode/molecule_find_best_state_path.eps}	
%	\caption{		
%		Algorithm from \cite{Levin2012} of finding the optimal state sequence given the two end-state and the total time.
%	}
%	\label{fig:vis_disease}
%\end{figure}

% ============================================

%\subsection{Search for maximum probability state sequences by discrete-time techniques}

% ================================================

\subsection{Search for maximum likelihood state and duration sequences}

\label{sec:decode_max_like}

In \cite{Perkins2009NIPS}, a trajectory of the CTMC is a sequence of states along with the dwell time in all but the last state: $U = (s_0, \tau_0, s_1, \tau_1, ..., s_{k-1}, \tau_{k-1}, s_k)$. This represents that the system enters state $s_0$ at the beginning and where it stays for $\tau_0$ time, then goes to $s_1$, and stays for $\tau_1$ and so on. 
	Eventually, the system hits state $s_k$ and remains there. Let $U_t = (s_0, \tau_0, s_1, \tau_1, ..., s_{k_t-1}, \tau_{k_t-1}, s_{k_t})$ be a random variable describing the trajectory of the system up until time $t$.
	This represents that there are $k_t$ state transitions up until time $t$, where $k_t$ itself is also a random variable.
	
	Given the initial state $s$, a total time $t$, the likelihood of a particular trajectory $U$ is shown as\ cite{}:
	\[L(U_t = U | s_0=s) = 
	\begin{cases} 0 & \mbox{if } s_0 \neq s \mbox{ or } \sum_{i=0}^{k-1} t_i > t \\ 
(\prod_{i=0}^{k-1} q_{s_i} e^{-q_{s_i} t_i} v_{s_i, s_{i+1}} ) (e^{-q_{s_k} (t - \sum_i \tau_i}) & \mbox{otherwise } \end{cases}  \]
The condition $\sum_{i=0}^{k-1} t_i > t$ in the first line means that the likelihood is zero if the chain has total time larger than $t$. Otherwise, in the second case
the first parenthesis $(\prod_{i=0}^{k-1} q_{s_i} e^{-q_{s_i} t_i} v_{s_i, s_{i+1}} )$ represents the likelihood of the dwell time until state $s_{k-1}$ and the state transitions in the sequence. The second parentheses $(e^{-q_{s_k} (t - \sum_i \tau_i})$ accounts for the probability that the dwell time in the last state does not finish before time $t$.

The end-conditioned most likely trajectory problem can be formulated as:
\[ arg~ max_U ~~ L(U_t = U | s(0)=s, s(t) = s^{'})  \]
where $s$ and $ s^{'}$ are the two given end-states, and $t$ is the given total time.\\

\begin{itemize}
\item \textbf{Find the most likelihood dwell time for a given state sequence:} 
	In this setting, the optimization problem becomes:
	\[ arg~ max_{(\tau_0, ..., \tau_{t_{k-1}})} ~~ L(U_t = U | s_0, s_1, ...., s_k)  \mbox{~~~~s.t.~~} \sum_i^{k-1} {t_i}< t \]
    
    In  \cite{Perkins2009NIPS}, it is shown that when given a particular state sequence, if state $s_i$ has the largest expected dwell time (i.e., has the smallest holding time parameter $q_i$), then the most likely setting of dwell time is derived by putting all of the time $T$ in state $s_i$ (the slowest state), and all other transitions happen instantaneously.
    This result is not unintuitive, but is dissatisfying in the sense that the resulting most likely set of dwell time is not typical, since none are close to their expected value.
    
\item    \textbf{Find the most likely state sequence for give end-states and total time:}	        
    With the solution for the above problem that all the times goes into the slowest state, one can now finds the most likely state sequence that maximize the likelihood using the derived formula:    
\[ arg~ max_{(\tau_0, ..., \tau_{k-1})} ~~ L(U_t = U | s_0 = s(0))  =  (\prod_{i=0}^{k-1} q_{s_i} e^{-q_{s_i} t_i} v_{s_i, s_{i+1}} ) e^{(min_{i=0}^k q_{s_i})t}. 
\]
    The solution can be found using dynamic programming. In order to build the maximum likelihood paths of increasing length, one finds the best ways of extending the shorter paths  \cite{Perkins2009NIPS}.
    The main difference here to other typical dynamic program problems is to remember not just the current score, the current end-state, but also the smallest holding time parameter $q$ along the path.
    The running time of this algorithm is $O(K|S|^3)$, where $K$ is the number of state jumps, which can be limited to be a preset value.
    
\item 	\textbf{Situations where maximum likelihood trajectory is not well-defined:}    
    It is analyzed in  \cite{Perkins2009NIPS} that if a CTMC has a cycle of states $(s_0, s1, ..., s_k = s_0)$ such that 
\[ \prod_{i=0}^{k-1} v_{s_i, s_{i+1}} q_{s_i} \geq 1 \],
     than maximum likelihood trajectories do not exist.
    A sequence of trajectories with ever-increasing likelihood can be found if the cycle is reachable. 
    Thus, before seeking the maximum likelihood trajectories from a starting state $s$, 
    one should check if the graph has a cycle having the stated property.
    This can be done by setting the weight as $log v_{s_1, s_2} q_{s_1}$ for the edge $s_1$ to $s_2$, and check whether the graph contains a positive-weight cycle, which needs polynomial time computations.
\end{itemize}
%considering all duration assignments

%====================================
\section{Computation of time-conditioned state sequence probability}

\label{sec:effi_statepath_prob}

Here, the goal is to compute the probability of a state sequence $G = (s_1, ..., s_n)$ given the total spanning time $t$. This can be formulated as:
\begin{align}
p( G = (s_1, ..., s_n) | t) = & (\prod_{i=1}^{n-1} v_{s_i, s_{i+1}} )  p( \sum_{i=1}^{n-1} \tau_i < t \leq \sum_{i=1}^n \tau_i | G = (s_1, ..., s_n))  
\end{align}
where $n$ is the length of $G$, $v_{s_i, s_{i+1}}$ is the state transition probability, and $\tau_i$ is the duration in each state $s_i$. 

Note that $p( \sum_{i=1}^{n-1} \tau_i \leq t \leq \sum_{i=1}^n \tau_i | G)$ can be evaluated using matrix exponential on an auxiliary $\hat{Q}$ matrix constructed using only the states along the state path (Eqn. (4)(5) in \cite{Hajiaghayi2014}). In detail, if $G = (s_1, \cdots, s_n)$, we construct an auxiliary $(n+1) \times (n+1)$ rate matrix $\hat{Q}$ as follows:
\begin{align}
\hat{Q} = \begin{bmatrix}
  -q_{s_1} & q_{s_1}  & 0            & \cdots &  0  & 0  \\
  0             & -q_{s_2} & q_{s_2} & \cdots &  0  & 0  \\    
  \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
  0 & 0 & 0 & \cdots & -q_(s_n) & q_{s_n} \\
  0 & 0 & 0 & \cdots & 0 & 0 \\
\end{bmatrix}_{(n+1)\times(n+1)}
\end{align}
where $q_{s_k} = \sum_{i, i \neq k} q_{s_k, s_i}$ is the holding time parameter of state $s_k$. This matrix has the structure that only the transition from $s_i$ to $s_{i+1}$ is set positive at the $(i,i+1)$ entry in $\hat{Q}$. It has be shown in \cite{Hajiaghayi2014} that
\begin{align}
p( \sum_{i=1}^{n-1} \tau_i \leq t \leq \sum_{i=1}^n \tau_i | G) =  (e^{\hat{Q}  t})_{1, n}
\end{align}
which is a matrix exponential operation on the auxiliary matrix $\hat{Q}$.

\textbf{Closed-form formulation for the $(1,n)$ entry of $e^{\hat{Q} t}$:}
We find that the $(1,n)$th entry of $e^{\hat{Q} t}$ has closed-form via \textit{Laplace transformation}\footnote{This is a collaborative work with Shuang Li and Le Song, who derive this exact closed-form.}. The results are as below (For notation simplicity, we write $q_{s_i}$ as $q_i$):

\begin{itemize}
	\item If $q_i, i = 1,...,n$ are distinct, we have
		\begin{align*}
		(e^{\hat{Q} t})_{1,n} =  \frac{1}{q_n}   \sum_{i=1}^n [ ( \prod_{j=1,j \neq i}^n \frac{q_j}{q_j - q_i} ) q_i e^{-q_i  t} ]
		\end{align*}				
	\item If $q_i, i = 1,...,n$ are not distinct, without loss of generality, we assume $q_1 = q_2 = ... = q_p$, and $q_{p+1} \neq q_{p+2} ... \neq q_n$, then we have the form below:
		\begin{align*}
		(e^{\hat{Q}  t})_{1,n} =  ( \frac{a_{11}}{(p-1)!} t^{p-1} + \frac{a_{12}}{(p-2)!} t^{p-2} + ... + a_{1p}) e^{-q_1 t} + A_{p+1} e^{-q_{p+1}t} + ... + A_n e^{-q_n t}		
		\end{align*}
\end{itemize}
Below we list some steps to derive $(e^{\hat{Q}  t})_{1,n}$ when $q_i$ are distinct using \textit{Laplace Transform} and the \textit{Inverse Laplace Transform} by \textit{Partial Fraction Expansion} as below:
\begin{align*}
	(e^{\hat{Q}  t})_{1,n} = \mathbb{F}^{-1} ( \mathbb{F}( (e^{\hat{Q}  t})_{1,n} ) )
\end{align*}
where $\mathbb{F}^{-1}$ is \textit{Laplace Transform} and $\mathbb{F}^{-1}$ is \textit{Inverse Laplace Transform}.
\begin{align*}
	\mathbb{F}(s) = \mathbb{F} (e^{\hat{Q}  t})_{1,n} = (sI - \hat{Q})^{-1}_{1,n} = \frac{q_1 q_2 ... q_{n-1}}{(s+q_1)(s+q_2)...(s+q_n)}
\end{align*}

If all  $q_i, i = 1,...,n$ are distinct, then we have
\begin{align*}
	\mathbb{F}(s) = \frac{A_1}{(s+q_1)} + \frac{A_1}{(s+q_2)} + ... + \frac{A_{n-1}}{(s+q_{n-1})} + \frac{A_{n}}{(s+q_{n})} (Partial~Fraction~Expansion)
\end{align*}
, where
\begin{align*}
A_i = lim_{s \rightarrow -q_i} (s+q_i) \mathbb{F}(s) = \frac{q_1 q_2 ... q_{n-1}}{(-q_i+q_1)...(-q_i+q_{i-1})(-q_i+q_{i+1})...(-q_i+q_n) }.
\end{align*}
Then we have
\begin{align*}
(e^{\hat{Q}  t})_{1,n} &= \mathbb{F}^{-1} ( \mathbb{F}(s)) 
= A_1 e^{-q_1 t} + A_2 e^{-q_2 t} + ... + A_n e^{-q_n t} \\
& = \frac{1}{q_n}   \sum_{i=1}^n [ ( \prod_{j=1,j \neq i}^n \frac{q_j}{q_j - q_i} ) q_i e^{-q_i  t} ]
\end{align*}

\subsection{Comparison of time complexity}

Here, we compare the time complexity of computing the state sequence probability given a total using a direct matrix exponential method and the closed-form expression we derived. The comparison is listed in Table \ref{table:time_path_prob}. The direct method means that to compute $(e^{\hat{Q}  t})_{1,n}$ by computing the matrix exponential and then read the $(1,n)$ entry, which needs $O(n^3)$ time. Clearly, our closed-form results only $O(n^2)$ time, but it need that all $q_i$ are distinct.

\begin{table*}[!htb]
	\centering	
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\caption{
		Time complexity comparison of all methods in evaluating time-conditioned path probability ($n$: number of states in the path)
	}	
	\begin{tabular}{|l||l||l|}
		\hline
		Complexity & direct-expm & Ours \\ \hline \hline
		Time & $O(n^3)$ & $O(n^2)$ \\ \hline \hline
		Prerequisite & none & $q_i$ distinct \\ \hline		
	\end{tabular}	 
	\label{table:time_path_prob}
\end{table*}

% =============================================
 
\section{Computation of path-and-time conditioned expected state duration}

\label{sec:effi_state_expect}

To the best of our knowledge, we have not found any literature that explicitly write down the closed-form and methods for computing expected state duration for a \textit{path-conditioned} CTMC. We derive a closed-form formulation for computing these path-conditioned statistics, which is applicable when $q_i$ for the states in the path are distinct. We also compare the time complexity of using our closed-form to using the three alternative methods (Expm, Unif, Eigen) which are originally used in end-state conditioned cases, to compute path-conditioned statistics by applying on an auxiliary matrix according to the state path.

%but fo apply on the auxiliary matrix constructed according to the state path.

% Here, our derivation of the expected state duration is inspired by the paper \cite{} % phase-type

We now explain our derived closed-form in detail\footnote{This is a collaborative work with Shuang Li and Le Song.}. Given a state sequence $G = (s_1, ..., s_n)$, a total duration $t$, the computation of the expected state duration $\tau_k$, for state $k = 1,...,n$ is as below:
\begin{align}
& E (\tau_k | G , \sum_{i=1}^{n-1} \tau_{i} \le t < \sum_{i=1}^{n} \tau_i ) 
= E [\int_{0}^{t} \mathbf{1} (S_u = s_k) du | G, \sum_{i=1}^{n-1} \tau_{i} \le t < \sum_{i=1}^{n} \tau_i  ] \\
&= \int_0^t p(S_u = s_k | G , \sum_{i=1}^{n-1} \tau_{i} \le t < \sum_{i=1}^{n} \tau_i ) du \\
&= \frac{\int_0^t (e^{\tilde{Q}_{k,A} u})_{1,k}  (e^{\tilde{Q}_{k,B} (t-u)})_{1,n-k+1} du}{ (e^{\tilde{Q} t})_{1,n}} \\
&= \frac{\int_0^t   [ a_{k,1}  e^{-q_1 u} + \cdots + a_{k,k} e^{-q_k u} ] \cdot [b_{k,k} e^{-q_k (t-u)} + \cdots + b_{k,n} e^{-q_n (t-u)}] du }{(e^{\tilde{Q} t})_{1,n}} \\
&=  \frac{( \sum_{i=1}^k \sum_{j=k, i \neq j}^{n} a_{k,i} b_{k,j} \frac{e^{-q_i t} - e^{-q_j t}}{-q_i + q_j}  ) + t (a_{k,k} b_{k,k}  e^{-q_k t})}{\frac{1}{q_n} \sum_{i=1}^{n} \bigg[ ( \prod_{j=1, j \neq i}^n \frac{q_j}{q_j-q_i} ) q_i e^{-q_i t} \bigg] }
\label{equ:tau}
\end{align}
where $q_i = \sum_{i \neq j} q_{ij}$ are the holding time parameters, $\tilde{Q}$ is the auxiliary matrix for the entire state path:
% Q
\begin{align}
\tilde{Q} & = \begin{bmatrix}
  -q_1 & q_1 & 0 & \cdots & 0 & 0 \\
  0 & -q_2 & q_2 & \cdots & 0 & 0 \\
  \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
  0 & 0 & 0 & \cdots & -q_n & q_n \\
  0 & 0 & 0 & \cdots & 0 & 0 \\
\end{bmatrix}_{(n+1)\times(n+1)},
\end{align}
, $\tilde{Q}_{k,A}$ is the auxiliary matrix for the partial state path from the first state to the $k$th state, 
% QA
\begin{align*}
%\footnotesize
\tilde{Q}_{k,A} = \begin{bmatrix}
  -q_1 & q_1 & 0 & \cdots & 0 & 0 \\
  0 & -q_2 & q_2 & \cdots & 0 & 0 \\
  \cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
  0 & 0 & 0 & \cdots & q_k & q_k \\
  0 & 0 & 0 & \cdots & 0 & 0 \\
\end{bmatrix}_{(k+1)\times(k+1)},
\end{align*}
, and $\tilde{Q}_{k,B}$ is the auxiliary matrix for the partial state path from the $(k+1)$th state to the last state (the $n$th state):
\begin{align*}
\tilde{Q}_{k,B} = \begin{bmatrix}
-q_k & q_k & 0 & \cdots & 0 & 0 \\
0 & -q_{k+1} & q_{k+1} & \cdots & 0 & 0 \\
\cdots & \cdots & \cdots & \cdots & \cdots & \cdots \\
0 & 0 & 0 & \cdots & -q_n & q_n \\
0 & 0 & 0 & \cdots & 0 & 0 \\
\end{bmatrix}_{(n-k+2)\times(n-k+2)}
\end{align*}
We also have the closed-form expression for $(e^{\tilde{Q} t})_{1,n}$ derived from the previous section as follows:
\begin{align}
& (e^{\tilde{Q} t})_{1,n} = \sum_{i=1}^{n} \bigg[ ( \prod_{j=1, j \neq i}^n \frac{q_j}{q_j-q_i} )  \frac{q_i}{q_n}  e^{-q_i T} \bigg] 
= \sum_{i=1}^{n} c_i e^{-q_i T}
\end{align}
where  $ c_i = ( \prod_{j=1, j \neq i}^n \frac{q_j}{q_j-q_i} )  \frac{q_i}{q_n}$. Finally, the terms $a_{k,i}$ and $b_{k,j}$ are defined as:
\begin{align}
\begin{cases}
a_{k,i} = \frac{q_i}{q_k}  (\prod_{m=1, m \neq i}^k \frac{q_m}{q_m - q_i})  &  k = 1, \cdots, n   ;  \text{  } i = 1, \cdots, k\\
b_{k,j} = \frac{q_j}{q_n}  (\prod_{m=k, m \neq j}^n \frac{q_m}{q_m - q_j}) & k = 1, \cdots, n ; \text{  }  j = k, \cdots, n \\ 
\end{cases}
\end{align}
which are derived from the closed-form expression for $(e^{\tilde{Q} t})_{1,n}$.

\textbf{Efficient computation of the expected duration for each state in the state path}:
we can derive the recursive relation between $a_{k,i}$ and $a_{k-1,i}$, and also $b_{k,j}$ and $b_{k+1,j}$, so that the computation of these coefficients can be efficient:
\begin{align}
\begin{cases}
a_{k,i} = a_{k-1,i} \frac{q_{k-1}}{q_k - q_i}  &  k = 1, \cdots, n   ;  \text{  } i = 1, \cdots, k\\
b_{k,j} = b_{k+1,j} \frac{q_{k}}{q_k - q_j} & k = 1, \cdots, n ; \text{  }  j = k, \cdots, n \\ 
\end{cases}
\end{align}

\textbf{Time complexity analysis:}
The time complexity in computing all $\tau_k$, $k=1,...,n$, where $n$ is the length of the inner path is $O(n^3 / 6)$. The detailed analysis is as follows. First,
the computation of all required $a_{k,i}$ and $b_{k,j}$ from the derived recursive form needs $O(n^2)$. Second, the computation of the common denumerator requires $O(n^2)$. Third, the computation of the numerator for one $\tau_k$ using the precomputed $a_{k,i}$ and $b_{k,j}$, requires  $k(n-k) = O(n^2)$. Finally, the computation of the numerator for all $\tau_k$ needs $\sum_{k=1}^n k(n-k) = (n^3-n)/6 = O(n^3/6)$.

Thus, evaluating just one expected state duration requires $O(n^2)$ computations, and evaluating all expected state durations along the path needs $O(n^3)$ ($n$ is the path length).

\subsection{Comparison of time complexity}

We compare the time complexity of computing the expected state durations given the state path and a total time from the three alternative methods (Expm, Unif, Eigen) and our closed-form solution. The three alternative methods \textit{(Expm, Unif, Eigen)} are originally used in computing the end-state conditioned statistics (see more details in Chapter 3). To use them for computing path-conditioned statistics, we only need to construct the auxiliary matrix $Q$ using the state path as the new rate matrix, and the remaining formulations are the same for calculating the end-state and path conditioned statistics. 

The time complexity comparison is listed in Table \ref{table:compare_time_expect_duration}. Our closed-form expression have only $O(n^2)$ time in computing one expected state duration, while all other methods require at least $O(n^3)$ as these alternative methods all involve matrix multiplications. When computing the expected duration for all states along the path, our close-form method has $O(n^3)$ complexity, and is more efficient than \textit{Expm and Unif} methods. However, our method and \textit{Eigen} both have prerequisite of its use, while \textit{Expm} and \textit{Unif} are more general.

%in evaluating path-and-time conditioned state expected duration}:

\begin{table*}[!htb]
	
	{\footnotesize
	\centering	
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\caption{
		Time complexity comparison of all methods in evaluating path-and-time conditioned expected state durations.
		(n: number of states in the path, $M$: the truncation point for \textit{Unif}, set as $\ulcorner 4 + 6 \sqrt{\hat{q} t} + (\hat{q} t) \urcorner$, where $\hat{q} = max_i ~q_i$ for states in the path, and $t$: the total time).
	}	
	\label{table:compare_time_expect_duration}
	\begin{tabular}{|l||l|l|l||l|}
		\hline
		Complexity & Expm & Unif & Eigen & Our Closed-Form \\ \hline \hline
		For one state & $O((2n)^3)$ & $O(M n^3 + M^2)$ & $O(n^3 + n^2)$ & $O(n^2)$  \\ \hline
		For all states & $O(n(2n)^3)=O(n^4)$ & $O(M n^3 + M^2 n)$ & $O(n^3 + n^3)$ & $O(n^3)$  \\ \hline \hline
		Prerequisite & none & none & Q diagonalizable & $q_i$ distinct \\ \hline		
	\end{tabular}	
	} 
	
\end{table*}

%\tabincell{c}{$O(\hat{M} S^3 + \min(rS^2, V) S M^2$ \\ + $\min(rS^2, V) L M^2)$} 

%=======================

% computing optimal state sequence and expected state duration

\section{An simulation example}

We now show one simulation example of computing the optimal state sequence given two end-states and a total time using the method from \cite{Levin2012} (Matlab and R package can be downloaded from the author's website), and then computing the expected state duration for each state in the optimal path using our presented closed-form and the three alternative methods (\textit{Expm, Unif, Eigen}).

In Fig.~\ref{fig:2_state_digraph}, we show a simple 2-state complete digraph models, with state $s_1$ has $q_1=1$ (mean holding time = 1) and $s_2$ has $q_2=0.5$ (mean holding time = 2). Now if we set the beginning state to be $s_1$, the terminating state to be $s_2$ and a total duration = $12$. What is the optimal state sequence considering all possible dwelling time assignments? 

The path extending and pruning method from \cite{Levin2012} gives the solution of the best state sequence as $(1,2,1,2,1,2,1,2)$, and our methods to compute expected state duration given the path and total time, gives the corresponding durations as $(1,2,1,2,1,2,1,2)$ which sums to 12. This result corresponds to our intuition of the best state path and the expected dwelling time of this model based on the holding time parameters $q_i$.

\begin{figure}[!t]
	\centering
	\includegraphics[width=5cm]{CTHMM_decode/small_cycle.eps}
	\caption{
	A simple 2-state digraph used to demonstrate the optimal state sequence decoding and computation of the expected state duration for the optimal path.
	}
	\label{fig:2_state_digraph}
\end{figure}

%============================================

\section{Experimental results in computing path-and-time conditioned expected state duration}

We test the running time of computing path-and-time conditioned expected state duration. Our setting is as follows. Given a state path of length $n$, each state's holding time parameter $q_i$ is generated randomly from $[0~1]$. The testing total time $T$ is set to be the sum of the mean holding time parameter $\sum_{i=1}^{n} 1/q_i$. We test the running time for $n = 20, 30, 40$, and for each testing, 10 runs are tested and the results are averaged. 

The running time results are listed in Table \ref{table:compare_runtime_expect_dur}. We find that $Eigen$ method tends to be the faster but fails often for $n$ is large. Our closed-form has better running time than Expm and Unif method in all testing cases. Unif method becomes slower when the total time $T$ is larger (when $n$ is large). This is due to its quadratic dependency of time. In terms of the accuracy results, we find that in our testing cases, all methods can derive similar expected state duration and the durations are sum to the total time, except the runs when Eigen method fails. However, note that our closed-form can only be used when each $q_i$ are distinct. Regarding to the generalizability and running time together, $Expm$ method appears to be the best choice.

\begin{table*}[!htb]
	\centering	
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\caption{
		Running time comparison of all methods in evaluating path-and-time conditioned expected state durations. For each setting, 10 random runs are tested and the average running time is reported.
	}	
	\begin{tabular}{|l||l|l|l||l|}
		\hline
		Time & Expm & Unif & Eigen & Our Closed-Form\\ \hline \hline
		$n = 20$ & 0.011 s & 0.375 s &  0.002 s & 0.005 s \\ \hline
		$n = 30$ & 0.029 s & 0.876 s &  0.007 s (fail: 1/10) & 0.016 s \\ \hline
		$n = 40$ & 0.061 s & 18.91 s &  0.012 s (fail: 5/10) & 0.030 s \\ \hline
%		$n = 50$ &  &  &  &  \\ \hline
	\end{tabular}	 
	\label{table:compare_runtime_expect_dur}
\end{table*}

% n = 20
%Eigen: 0 minutes and 0.002252 seconds
%Closed-Form: 0 minutes and 0.005608 seconds
%Expm: 0 minutes and 0.010541 seconds
%Unif: 0 minutes and 0.375448 seconds
%
%% n = 30
%eigen_num_fail = 1
%Eigen: 0 minutes and 0.006930 seconds
%Closed-Form: 0 minutes and 0.015911 seconds
%Expm: 0 minutes and 0.028837 seconds
%Unif: 0 minutes and 0.875968 seconds
%
%% n = 40
%eigen_num_fail = 5
%Eigen: 0 minutes and 0.011635 seconds
%Closed-Form: 0 minutes and 0.029932 seconds
%Expm: 0 minutes and 0.061457 seconds
%Unif: 0 minutes and 18.906624 seconds

%============================================

\section{Conclusion and future work}

In this chapter, we review the prior works for CTMC and CT-HMM in finding the optimal state sequence considering all possible duration assignments given two fixed end-states and a total time. Another related problem is to find the maximum likely state and duration sequence together under same conditions. It is found that the former problem setting can result in more biological meaningful solution, while the solution derived from the latter setting gives all duration to the state with the largest mean holding time (smallest $q_i$), which is usually undesirable in practice. The exact solution found for the first problem can be useful in real applications to understand the best hidden path. However, the prior work didn't present the method to compute the expected duration for the found optimal state path.

%Design a pruning criteria that can prune paths during search. But the testing is itself time consuming. The method can result in exhaustive search if no path can be pruned. In addition, the author doesn’t present how to assign expected duration once an optimal state path is found.

To the best of our knowledge, we are the first to explicitly tackle the problem of computing the path-and-time-conditioned expected state durations. While the techniques for finding end-state conditioned expectations can be applied for the path-conditioned one, by working on the auxiliary matrix constructed for the path, the resulting computation may not be the most efficient. We derive the exact closed-form for computing the following two statistics without using any matrix multiplications but with the prerequisite that $q_i$ in the paths are all distinct. The two statistics are (1) the probability of a state sequence given a total time, computed in $O(n^2)$, (2) the expected state duration given a state sequence and a total time, computed in $O(n^2)$  for just one state, and $O(n^3)$ for all states along the path. We also compare the time complexity of using \textit{Expm, Unif, Eigen} methods to the newly-derived closed-form. The former three methods require at least $O(n^3)$ for just one state, because these methods all require matrix multiplication. The derived new closed-form expression, which is more time efficient, can be useful in CTMC and CT-HMM decoding and inference tasks. 

%We fill the gap

==> EM.tex <==
\subsection{EM Algorithms for CT-HMM}
\label{sec:em}

Pseudocode for the EM algorithm for CT-HMM parameter learning is shown in Algorithm~\ref{alg:em-outerloop}. Multiple variants of the basic algorithm are possible, depending upon the choice of method for computing the end-state conditioned expectations, along with the choice of \emph{hard} or \emph{soft} decoding for obtaining the posterior state probabilities in Eq.~\ref{eq:inHMM}. %Note that in line 7 of Algorithm~\ref{alg:em-outerloop}, we group probabilities from successive visits of same time interval and the same specified end-states in order to save computation time.
%This is valid because in a time-homogeneous CT-HMM, $\mathbb{E}[n_{ij}|s(t_{v}) = k,s(t_{v+1})=l,\hat{Q}_{0}] = \mathbb{E}[n_{ij}|s(0) = k,s(\tau_{v})=l,\hat{Q}_{0}]$, where $\tau_{v}=t_{v+1} - t_v$, so that the expectations only need to be evaluated for each distinct time interval, rather than each different visiting time (also see the discussion below Eq.~\ref{equ:L}).

The remaining step in finalizing the EM algorithm is to discuss the computation of the end-state conditioned expectations (ESCE) for $n_{ij}$ and $\tau_i$ from Eqs.~\ref{eq:endn} and~\ref{eq:endt}, respectively.  The first step is to express the expectations in integral form, following~\cite{Hobolth2005}:
\begin{align}
& \mathbb{E}[n_{ij} | s(0)= k, s(t) = l,Q]
=  \frac{q_{i,j}  }{P_{k,l}(t)}
\int_{0}^{t} P_{k,i}(x) P_{j,l}(t-x)\, dx\label{eq:nij}
\\
& \mathbb{E}[\tau_{i} | s(0)= k, s(t) = l, Q]
=  \frac{1}{P_{k,l}(t)}  \int_{0}^{t} P_{k,i}(x) P_{i,l}(t-x)\, dx.\label{eq:taui}
\end{align}
From Eq.~\ref{eq:nij}, we define
$\tau_{k,l}^{i,j}(t) = \int_{0}^{t} P_{k, i}(x) P_{j,l}(t - x)dx = \int_{0}^{t} (e^{Qx})_{k,i} (e^{Q(t-x)})_{j,l}\, dx$, 
while $\tau_{k,l}^{i,i}(t)$ can be similarly defined for Eq.~\ref{eq:taui} (see~\cite{nodelman05} for a related construction). Three primary methods for computing $\tau_{k,l}^{i,j}(t)$ and $\tau_{k,l}^{i,i}(t)$ have been proposed in the CTMC literature: an eigendecomposition based method, which we refer to as \emph{Eigen}, a method called \emph{uniformization} (\emph{Unif}), and a method from~\cite{VanLoan1978} for computing integrals of matrix exponentials, which we call \emph{Expm}.  \emph{Eigen} and \emph{Unif} both involve expressing the terms $P_{k, i}(x) P_{j,l}(t - x)$ as summations and then integrating the summations.  Eigen utilizes an eigendecomposition-based approach, while Unif is based on series approximations.  \emph{Expm} notes a connection between the integrals and a system of differential equations, and solves the system.  We describe each method,  show how to improve the complexity of the \emph{soft Eigen} method, and discuss their tradeoffs.  

\begin{algorithm}[t]
	\caption{CT-HMM Parameter Learning (Soft/Hard)}
	\label{alg:em-outerloop}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} data $O=(o_0, ..., o_V)$ and $T=(t_0,\ldots, t_V)$, state set $S$, edge set $L$, initial guess of $Q$ 
		\STATE {\bfseries Output:} transition rate matrix $Q = (q_{ij})$    
		\STATE Find all time intervals between events $\tau_{v}=t_{v+1}-t_{v}$ for $v=1,...,V-1$, where $t_{1}=t_{0}=0$
		\STATE Compute  $P(\tau_{v})=e^{Q\tau_{v}}$ for each $\tau_{v}$   
		\REPEAT      
		\STATE Compute $p(v,k,l)=p(s(t_v)=k, s(t_{v+1})=l | O, T, Q)$ for all $v$,  and the complete/state-optimized data likelihood $l$ by using Forward-Backward (soft) or Viterbi (hard) 
		\STATE Use \emph{Expm, Unif} or \emph{Eigen} method to compute $\mathbb{E}[n_{ij}|O, T, Q]$ and $\mathbb{E}[\tau_i|O, T, Q]$
		\STATE Update $q_{ij} = \frac{\mathbb{E}[n_{ij}|O, T, Q]}{ \mathbb{E}[\tau_i|O, T, Q]}$, and $q_{ii} = -\sum_{i \neq j} q_{ij}$   
		\UNTIL{likelihood $l$ converges}
	\end{algorithmic}
\end{algorithm}

Across the three methods, the bottleneck is generally matrix operations, particularly matrix multiplication.  Our finding is that with our improvements, \emph{soft Eigen} is the preferred method except in the case of an unstable eigendecomposition.  It is efficient due to having few matrix multiplications and it is accurate due to being a soft method.  We find in our experiments that it is very fast (see Fig. \ref{fig:bar-chart-all}) and that the stability of \emph{Eigen} is usually not a problem when using random initialization.  However, in the case where \emph{Eigen} is unstable in any iteration, the alternatives are \emph{soft} Expm, which has the advantage of accuracy, and \emph{hard} Unif, which is often faster.  Note that one can switch back to \emph{Eigen} again once the likelihood is increasing.

\subsubsection{The Eigen Method}

The calculation of the ESCE $\tau_{k,l}^{i,i}(t)$ and
$\tau_{k,l}^{i,j}(t)$
can be done in closed-form if $Q$ can be diagonalized via its eigendecomposition (the \emph{Eigen} method of \cite{Metzner2007} and \cite{MetznerJournal2007}). Consider the eigendecomposition
$Q = U D U^{-1}$, 
where the matrix $U$ consists of all eigenvectors associated with the corresponding eigenvalues of $Q$ in the diagonal matrix $D=diag(\lambda_1, ...,\lambda_n)$.  Then we have $e^{Qt} = U e^{Dt} U^{-1}$
and the integral can be written as:
%
\begin{align}
\tau_{k,l}^{i,j}(t) 
= \sum_{p=1}^{n} U_{kp} U_{pi}^{-1} \sum_{q=1}^{n} U_{jq} U_{ql}^{-1} \Psi_{pq}(t)
\end{align}
%
where the symmetric matrix $\Psi(t)=[\Psi_{pq}(t)]_{p,q \in S}$ is defined as:
%
\begin{align}
\Psi_{pq}(t) = \begin{cases}
t e^{t \lambda_p} \text{~~if~} \lambda_p = \lambda_q\\
\frac{e^{t \lambda_p} - e^{t \lambda_q}}{\lambda_p - \lambda_q} \text{~~if~} \lambda_p \neq \lambda_q\label{eq:eigen-method-inner-element}
\end{cases}
\end{align}
%
We now describe a method for vectorizing the \emph{Eigen} computation, which results in improved complexity in the \emph{soft} case.  Let $V=U^{-1}$, $\circ$ be the Hadamard (elementwise) product, and $V_{i}^{T}$ refer to the $i$th column of $V$, and $U_{j}$ the $j$th row of $U$, then
%
\begin{align}
\tau_{k,l}^{i,j}(t)&=[U[V^{T}_{i}U_{j}\circ \Psi]V]_{kl}\label{eq:vector-eigen}
\end{align}
%
This allows us to perform only one matrix construction for all $k,l$, but still requires two matrix multiplications for each $ij$ with an allowed transition or edge.\footnote{Note that a version of equation \ref{eq:vector-eigen} appears in~\cite{Metzner2007}, but that version contains a small typographic error.}

We now show how to reuse the matrix-matrix products across edges and replace them by a Hadamard product to improve efficiency further.  A similar idea was explored in~\cite{mcgibbon2015efficient}, but their derivation is for the gradient calculation of a CTMC, which we extend to EM for CT-HMMs.  The intuition is that since matrix multiplication is expensive, by rearranging matrix operations, we can do one matrix multiplication, cache it, and reuse it so that we only do elementwise matrix products for every possible transition combination $i$ and $j$, rather than doing matrix multiplications for every such combination.

Let $F$ be a matrix given by $F_{kl}=\frac{p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0})}{P_{kl}(t)}$, and let $A^{ij}=V^{T}_{i}U_{j}\circ \Psi$.  Then
%
\begin{align}
\sum_{k,l=1}^{|S|}p(s(t_{v})=k,s(t_{v+1})=l|&O,T,\hat{Q}_{0})\mathbb{E}[n_{ij}|s(t_{v})=k,s(t_{v+1})=l,\hat{Q}_{0}]\\
&=q_{ij}\sum_{k,l=1}^{|S|}([U[V^{T}_{i}U_{j}\circ \Psi]V]\circ F)_{kl}\\
&=q_{ij}\sum_{k,l=1}^{|S|}([UA^{ij}V]\circ F)_{kl}
\end{align}
%
Now note these two properties of the trace and Hadamard product, which hold for any matrices $A,B,C,D$:
%
\begin{align}
\sum_{ij}(A\circ B)_{ij}&=\text{Tr}(AB^{T})\\
\text{Tr}(ABCD)&=\text{Tr}(BCDA)
\end{align}
%
Then
%
\begin{align}
\sum_{k,l=1}^{|S|}([UA^{ij}V]\circ F)_{kl}&=\text{Tr}(UA^{ij}VF^{T})\\
&=\text{Tr}(A^{ij}VF^{T}U)\\
&=\sum_{kl}(A^{ij}\circ (VF^{T}U)^{T})_{kl}\\
&=\sum_{kl}(A^{ij}\circ \underbrace{(U^{T}FV^{T})}_{\text{reuse}})_{kl}\label{eq:reuse}
\end{align}
%
The term $U^{T}FV^{T}$ is not dependent on $i,j$: only $A^{ij}$ is, and $A^{ij}$ does not require any matrix products to construct.  Thus for each event or time interval, the na\"ive implementation of Eq. \ref{eq:vector-eigen} required two matrix products for each $i,j$ that form an edge. Through the preceding construction, we can reduce this to only two matrix products in total.  We replaced all the other matrix products with Hadamard products.  This improves the complexity by a factor of $S$, the number of states.  The case for the ESCE of the duration $\tau_{i}$ is similar.  Letting $A^{i}=V_{i}^{T}U_{i}\circ\Psi$ and using the subscript $v$ to denote the matrix constructed for observation $v$, the final expectations are
%
\begin{align}
E[n_{ij}|O,T,\hat{Q}_{0}]&=q_{ij}\sum_{v=1}^{V-1}\sum_{kl}(A^{ij}_{v}\circ (U^{T}F_{v}V^{T}))_{kl}\label{eq:efficientN}\\
E[\tau_{i}|O,T,\hat{Q}_{0}]&=\sum_{v=1}^{V-1}\sum_{kl}(A^{i}_{v}\circ (U^{T}F_{v}V^{T}))_{kl}\label{eq:efficientT}
\end{align}
%
Note that the \emph{Hard} eigen method avoids explicitly summing over all $k$ and $l$ states. The key matrix manipulation then is the construction of matrices where the rows and columns correspond to $k$ and $l$, respectively. Therefore, \emph{hard} eigen has the same complexity as \emph{soft} eigen when it is formulated as in Eqs.~\ref{eq:efficientN} and~\ref{eq:efficientT}. Thus, \emph{soft} eigen is the preferred choice.

{\bf Computing the ESCE using the \emph{Eigen} method} Algorithm \ref{alg:scale-eigen} presents pseudocode for our \emph{Eigen} method using the Hadamard product and trace manipulations.  The algorithm does two matrix multiplications for each observation, and does only Hadamard products for each state and edge after that.

\begin{algorithm}
\caption{Eigen Algorithm for ESCE}
\label{alg:scale-eigen}
\begin{algorithmic}[1]
\STATE Perform eigendecomposition $Q=UDV$ using balancing, where $V=U^{-1}$
\FOR{$v=1$ to $V-1$}
\STATE Compute $\tau_{v}=t_{v+1}-t_{v}$, set $t=\tau_{v}$
\STATE Compute $\Psi$ with $t=\tau_{v}\Rightarrow O(S^{2})$
\STATE Compute $F_{k,l}=\frac{p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0})}{P(t)}$
\STATE Compute $B=U^{T}FV^{T}$
\FOR{each state $i$ in S}
\STATE $A=V_{i}^{T}U_{i}\circ \Psi$
\STATE $E[\tau_{i}|O,T,Q]+=\sum_{k,l=1}^{|S|}(A\circ B)_{kl}\Rightarrow O(S^{2})$
\ENDFOR
\FOR{each edge $(i,j)$ in $L$}
\STATE $A=V_{i}^{T}U_{j}\circ \Psi\Rightarrow O(S^{2})$
\STATE $\mathbb{E}[n_{ij}|O,T,Q]+=q_{ij}\sum_{k,l=1}^{|S|}(A\circ B)_{kl}\Rightarrow O(S^{2})$
\ENDFOR 
\ENDFOR
\end{algorithmic}
\end{algorithm}


\subsubsection*{Stability of the Eigen Method}
In general, \emph{soft Eigen} is the fastest soft method, but $Qt$ can suffer from an ill-conditioned eigendecomposition which can prevent the method from being usable.
%%\footnote{In theory $Qt$ could be non-diagonalizable, but it is well known that the set of such matrices has measure $0$}.
In prior CTMC works~(\cite{Metzner2007,MetznerJournal2007}), they mention that the eigendecomposition can potentially be ill-conditioned, but do not characterize the scope of this problem, which we discuss now in more detail. Both the eigenvalue and eigenvector estimation problems can be ill-conditioned. For the eigenvalue problem, the primary issue is the condition number of the eigenvector matrix. This follows from the Bauer-Fike Theorem~(\cite{bauer1960norms}), which gives a bound on the error in estimating the eigenvalues (as a result of a perturbation $\Delta Q$ of the $Q$ matrix):
\begin{align}
\min_{\lambda\in \lambda(Q)}|\lambda-\mu|&\leq ||U||\cdot ||\Delta Q|| \cdot||U^{-1}||\\
&=\kappa(U)||\Delta Q||.
\end{align}
The error between an eigenvalue $\mu$ of $Q+\Delta Q$ and the true eigenvalue $\lambda$ is bounded by the matrix norm of the perturbation, $||\Delta Q||$, and the condition number $\kappa(U)$ of the eigenvector matrix $U$ of $Q$. We now discuss the impact of each of these two terms. The perturbation of $Q$, $||\Delta Q||$, is often due to rounding error and thus depends on the norm of $Q$.  A class of methods known as balancing or diagonal scaling due to~\cite{osborne1960pre} can help reduce the norm of $Q$. In our experiments, balancing did not provide a significant improvement in the stability of the eigendecomposition, leading us to conclude that rounding error was not a major factor. The condition number $\kappa(U)$ captures the structural properties of the eigenvector matrix. We found empirically that certain pathological structures for the $Q$ matrix, such as sparse triangular forms, can produce poor condition numbers. We recommend initializing the $Q$ matrix at the start of EM with randomly-chosen values in order to prevent the inadvertent choice of a poorly-conditioned $U$. We found that uniform initialization, in particular, was problematic, unless random perturbations were added.

Having discussed the eigenvalue case, we now consider the case of the eigenvectors.  For an individual eigenvector $r_{j}$, the estimation error takes the form
%
\begin{align}
\Delta{r}_{j}&=\sum_{k\neq j}\frac{l_{k}\Delta{Q}r_{j}}{\lambda_{j}-\lambda_{k}}r_{k}+O(||\Delta Q||^{2}),
\end{align}
%
where $l_{k}$ are left eigenvectors, $r_{j}$ and $r_{k}$ are right eigenvectors, and $\lambda_{j},\lambda_{k}$ are eigenvalues of $Q$ (see \cite{bindel2009principles} for details). Thus the stability of the eigenvector estimate degrades when eigenvalues are closely-spaced, due to the term $\lambda_{j}-\lambda_{k}$ in the denominator. Note that this condition is problematic for the ESCE computation as well, as can be seen in Eq.~\ref{eq:eigen-method-inner-element}. As was the case for the eigenvalue problem, care should be taken in initializing $Q$. 

In summary, we found that randomly initializing the $Q$ matrix was sufficient to avoid problems at the start of EM. While it is difficult in general to diagnose or eliminate the possibility of stability problems during EM iterations, we did not encounter any significant problems in using the \emph{Eigen} approach with either a uniform perturbation plus random noise or simply random initializations in our experiments. We recommend monitoring for a decrease in the likelihood and switching to an alternate method for that iteration in the event of a problem.  One can switch back to \emph{Eigen} once the likelihood is increasing again.

%%  Thus, eigenvector estimates are also sensitive to the matrix norm $||Q||$, but additionally are sensitive to  the term $l_{k}\Delta{Q}r_{j}$ and to close eigenvalues.
%% In light of this analysis, when using \emph{Eigen} we recommend starting with a random initialization and checking whether the likelihood decreases in any iteration.  We find that \emph{Eigen} is successful for all of our experiments.
%% We now discuss the issue more deeply and connect with the numerical linear algebra literature.  Given that there are several potential sources of instability, one should monitor that the likelihood is increasing at every iteration, and if it is not, one should switch to another method. 
%%  The main issue for the eigenvalues is the condition number of the eigenvector matrix, and the potential issue for the eigenvectors is close eigenvalues.  Note that if the difference in a pair of eigenvalues is small, the term for  $\lambda_p\neq \lambda_q$ in Eq. \ref{eq:eigen-method-inner-element} will blow up.
%% For the eigenvalue estimates, note the following theorem from \cite{bauer1960norms}, which says that the error in estimating a single eigenvalue has two terms in its bound: the linear-systems condition number of the eigenvector matrix, and a term that is related to the norm of the matrix.
%% \textbf{Theorem (Bauer-Fike):}
%% For matrix and vector norms, if $\mu$ is an eigenvalue of $||Q+\Delta Q||$, where $\Delta Q$ is a perturbation of $Q$, $U$ is the matrix of eigenvectors of $Q$, and $\lambda(Q)$ is the set of eigenvalues of $Q$, then
%% %
%% \begin{align}
%% \min_{\lambda\in \lambda(Q)}|\lambda-\mu|&\leq ||U||\cdot ||\Delta Q|| \cdot||U^{-1}||\\
%% &=\kappa(U)||\Delta Q||
%% \end{align}
%% %
%% where $\kappa(U)$ is the condition number of the eigenvector matrix of $Q$.  This says that, given some eigenvalue $\mu$ of the perturbed matrix, the Euclidean distance from it to the closest (hence the min) eigenvalue of the original matrix has the upper bound given.  Since we can upper bound the error of each eigenvalue estimate $\mu$, we can get the upper bound for all eigenvalues.
%% The important question then is: if either term is large, can we reduce it?  The perturbation of $Q$, $||\Delta Q||$, is often due to rounding error and thus depends on the norm of $Q$.  A class of methods known as balancing or diagonal scaling $\cite{osborne1960pre}$ can help with reducing the norm of $Q$, but these methods offer no guarantees for the condition number of the eigenvector matrix.  It is difficult to say intuitively when the condition number of the eigenvector matrix will be large.

\subsubsection{Expm Method}

Having described an eigendecomposition-based method for computing the ESCE, we now describe an alternative approach based on a classic method of ~(\cite{VanLoan1978}) for computing integrals of matrix exponentials. In this approach, an auxiliary matrix $A$ is constructed as 
$A = \begin{bmatrix} Q & B\\ 0 & Q \\ \end{bmatrix}$, where $B$ is a matrix with identical dimensions to $Q$. It is shown in~\cite{VanLoan1978} that
%
\begin{align}
\int_0^t e^{Qx} B e^{Q(t-x)} dt = (e^{At})_{(1:n), (n+1):(2n)}
\end{align}
%
where $n$ is the dimension of $Q$.  That is, the integral evaluates to the upper right quadrant of $e^{At}$.  Following~\cite{Hobolth2011}, we set $B = I(i, j)$, where $I(i,j)$ is the matrix with a $1$ in the $(i,j)$th entry and $0$ elsewhere. Thus the left hand side reduces to $\tau_{k,l}^{i,j}(t)$ for all $k, l$ in the corresponding matrix entries, and we can leverage the substantial literature on numerical computation of the matrix exponential. We refer to this approach as \emph{Expm}, after the popular Matlab function.  This method can be seen as expressing the integral as a solution to a differential equation.  See Sec. 4 of  \cite{Hobolth2011} for details.

The most popular method for calculating matrix exponentials is the Pad\'e approximation. As was the case in the \emph{Eigen} method, the two issues governing the accuracy of the Pad\'e approximation are the norm of $Q$ and the eigenvalue spacing. If the norms are large, scaling and squaring, which involves exploiting the identity $e^A=(e^{A/m})^m$ and using powers of two for $m$, can be used to reduce the norm. To understand the role of Eigenvalue spacing, consider that the Pad\'e approximation involves two series expansions $N_{pq}(Qt)$ and $D_{pq}(Qt)$, which are used to construct the matrix exponential as follows:
%
\begin{align}
e^{Qt}\approx[D_{pq}(Qt)]^{-1}N_{pq}(Qt)
\end{align}
%
When the eigenvalue spacing \emph{increases}, $D_{pq}(Qt)$ becomes closer to singular, causing large errors as described in~\cite{moler1978nineteen,moler2003nineteen}.

The maximum separation between the eigenvalues is bounded by the Gershgorin Circle Theorem(~\cite{golub2012matrix}), which states that all of the eigenvalues of a rate matrix lie in a circle in the complex plane centered at the largest rate, with radius equal to that rate.  That is, all eigenvalues $\lambda\in \lambda(Q)$ lie in $\{z\in \mathbb{C}:|z-\max{q_{i}}|\leq \max{q_{i}}\}$.  
%%In order to satisfy this, the real parts of the eigenvalues will always be negative or $0$.
This construction allows us to bound the maximum eigenvalue spacing of $Qt$ (considered as a rate matrix). Two eigenvalues cannot be further apart than twice the absolute value of the largest magnitude diagonal element.  Further, scaling and squaring helps with this issue, as it reduces the magnitude of the largest eigenvalue.  Additional details can be found in~(\cite{moler1978nineteen,moler2003nineteen,Higham2008}).

Because scaling and squaring can address stability issues associated with the Pad\'e method, we conclude that \emph{Expm} is the most stable method for computing the ESCE.  However, we find it to be dramatically slower than \emph{Eigen} (especially given our vectorization and caching improvements), and so it should only be used if \emph{Eigen} fails.

The \emph{Expm} algorithm does not have an obvious hard variant.  Hard variants involve calculating expectations conditioned on a single start state $k$ and end-state $l$ for the interval between the observations.  However, \emph{Expm}, by virtue of using the Pad\'e approximation of the matrix exponential, calculates it for all $k$ and $l$.  The output of the matrix exponential gives a matrix where each row corresponds to a different $k$ and each column a different $l$.  Developing a hard variant would thus require a method for returning a single element of the matrix exponential more efficiently than the entire matrix.  One direction to explore would be the use of methods to compute the action of a matrix exponential $e^{At}x$, where $x$ is a vector with a single $1$ and $0$'s elsewhere, without explicitly forming $e^{At}$ (see~\cite{al2011computing}).

{\bf Computing the ESCE using the \emph{Expm} method}
Algorithm \ref{alg:soft-soft-expm} presents pseudocode for the \emph{Expm} method for computing end-state conditioned expectations. The algorithm exploits the fact that the $A$ matrix does not change with time $t$. Therefore, when using the \emph{scaling and squaring} method~(\cite{Higham2008}) for computing matrix exponentials, one can easily cache and reuse the intermediate powers of $A$ to efficiently compute $e^{At}$ for different values of $t$.

\begin{algorithm}[h]
	\small
	\caption{Expm Algorithm for ESCE}
	\label{alg:soft-soft-expm}
	\begin{algorithmic}[1]
    	\FOR{$v=1$ {\bfseries to} $V-1$}
        \STATE $\tau_{v}=t_{v+1}-t_{v}$, set $t=\tau_{v}$
		\FOR{each state $i$ in $S$}
		\STATE $D_i = \frac{(e^{At})_{(1:n), (n+1):(2n)}}{P_{kl}(t)}$, where \small{$A = \begin{bmatrix} Q & I(i,i) \\ 0 & Q \\ \end{bmatrix}$ }

		\STATE $\mathbb{E}[\tau_i|O, T, Q]~+=~ \sum_{(k,l) \in L} p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0})  (D_i)_{k,l} $ 
		\ENDFOR
		\FOR{each edge ($i,j$) in $L$}
		\STATE $N_{ij} = \frac{q_{ij} (e^{At})_{(1:n), (n+1):(2n)}}{P_{kl}(t)}$, where \small{$A = \begin{bmatrix} Q & I(i,j) \\ 0 & Q \\ \end{bmatrix}$ } 

		\STATE $\mathbb{E}[n_{ij}|O, T, Q]~ += \sum_{(k,l) \in L} p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0})  (N_{ij})_{k,l} $ 
		\ENDFOR
		\ENDFOR  
	\end{algorithmic}
\end{algorithm}


\subsubsection{Uniformization}
We now discuss a third approach for computing the ESCE.  This was first introduced by ~\cite{Hobolth2011} for the CTMC case, and is called \emph{uniformization} (\emph{Unif}).  \emph{Unif} is an efficient approximation method for computing the matrix exponential $P(t) = e^{Qt}$(~\cite{Jensen1953,Hobolth2011}). It gives an alternative description of the CTMC process and illustrates the relationship between CTMCs and DTMCs (see \cite{RossBook1983}).  The idea is that instead of describing a CTMC by its rate matrix, we can subdivide it into two parts: a Poisson process $\{N(t):t\geq 0\}$ with mean $\hat{q}$, where $N(t)$ refers to the number of events under the Poisson process at time $t$, and a DTMC and its associated transition matrix $R$.  The state of the CTMC at time $t$ is then equal to the state after $N(t)$ transitions under the DTMC transition matrix $R$.  In order to represent a CTMC this way, the mean of the Poisson process and the DTMC transition matrix must be selected appropriately.

Define $\hat{q} = \max_i q_i$, and matrix $R = \frac{Q}{\hat{q}} + I$, where $I$ is the identity matrix. Then,
%
\begin{align}e^{Qt} = e^{\hat{q}(R-I)t} = \sum_{m=0}^{\infty} R^m \frac{(\hat{q} t)^m}{m!} e^{-\hat{q} t} 
= \sum_{m=0}^{\infty} R^m Pois(m ; \hat{q} t),
\end{align}
%
where $Pois(m; \hat{q} t)$ is the probability of $m$ occurrences from a Poisson distribution with mean $\hat{q} t$.  The expectations can then be obtained by directly inserting the $e^{Qt}$ series into the integral: 
%
\begin{align}
E[\tau_i| s(t) = l, s(0) = k] &= \sum_{m=0}^{\infty} \frac{t}{m+1} [ \sum_{n=0}^{m} (R^n)_{ki} (R^{m-n})_{il} ] Pois(m; \hat{q} t)\\
E[n_{ij}| s(t) = l, s(0) = k] &= R_{ij}
\sum_{m=1}^{\infty}   [ \sum_{n=1}^{m} (R^{n-1})_{ki}  (R^{m-n})_{jl} ] Pois(m; \hat{q} t)
\end{align}
%
The main difficulty in using \emph{Unif} in practice lies in determining the truncation point for the infinite sum. However, for large values of $\hat{q} t$, we have $Pois(\hat{q} t) \approx \mathcal{N}(\hat{q} t, \hat{q} t)$, where $\mathcal{N}(\mu, \sigma^2)$ is the normal distribution and one can then bound the truncation error from the tail of Poisson by using the cumulative normal distribution~(\cite{TataruBio2011}). Our implementation uses a truncation point at $M = \ulcorner 4 + 6 \sqrt{\hat{q} t} + (\hat{q} t) \urcorner$, which is suggested in~(\cite{TataruBio2011}) to have error bound of $10^{-8}$.

{\bf Computing the ESCE using the \emph{Unif} method} Algorithm~\ref{alg:unif} presents pseudocode for the \emph{Unif} method for computing end-state conditioned expectations. The main benefit of \emph{Unif} is that the $R$ sequence ($R,  R^2,...,R^{\hat{M}}$) can be precomputed (line 2) and reused, so that no additional matrix multiplications are needed to obtain all of the expectations. One main property of \emph{Unif} is that it can evaluate the expectations for only the two specified end-states, and it has $O(M^2)$ complexity, which is not related to $S$ (when given the precomputed $R$ matrix series).

%%In hard EM, many of the $p(s(t_v)=k, s(t_{v+1})=l | O, T, \hat{Q}_0)$ evaluate to $0$, and thus hard EM is more time efficient than soft EM. 
One downside of \emph{Unif} is that if $\hat{q_i} t$ is very large, so is the truncation point $M$.  The computation can then be very time consuming. We find that \emph{Unif}'s running time performance depends on the data and the underlying Q values. The time complexity analysis is detailed in Algorithm \ref{alg:unif} line 15.  This shows that the complexity of \emph{soft Unif} is unattractive, while \emph{hard Unif} may be attractive if \emph{Eigen} fails due to instability.

\begin{algorithm}[!ht]
	\caption{Unif Algorithm for ESCE}  
	\label{alg:unif}
	\begin{algorithmic}[1]
		\STATE Set $\hat{t} = max ~t_\Delta$; set $\hat{q} = max_i q_i$.
		\STATE Let $R = Q/\hat{q} + I$. Compute $R, R^2,...,R^{\hat{M}}$, $\hat{M} = \ulcorner 4 + 6 \sqrt{\hat{q} \hat{t}} + (\hat{q} \hat{t}) \urcorner$ $\Rightarrow O(\hat{M} S^3)$

		\FOR{$v=1$ {\bfseries to} $V-1$}
        \STATE $\tau_{v}=t_{v+1}-t_{v}$, set $t = \tau_{v}$
		\STATE $M = \ulcorner 4 + 6 \sqrt{\hat{q} t } + (\hat{q} t) \urcorner$; 
		\FOR{each state $i$ in $S$}
		\STATE $ E[\tau_i | s(0) = k, s(t) = l, Q] =
		\frac{\sum_{m=0}^M \frac{t}{m+1} [ \sum_{n=0}^{m} (R^n)_{ki} (R^{m-n})_{il} ] Pois(m; \hat{q} t)}{P_{kl}(t)}  $
		$\Rightarrow O(M^2)$
		\STATE  $E[\tau_i|O, T, Q] +=p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0}) E[\tau_i | s(0) = k, s(t) = l] $   
		\ENDFOR           
		\FOR{each edge $(i,j)$ in $L$}      
		\STATE $ E[n_{ij} | s(0) = k, s(t) = l, Q] = \frac{R_{ij} \sum_{m=1}^M   [ \sum_{n=1}^{m} (R^{n-1})_{ki}  (R^{m-n})_{jl} ] Pois(m; \hat{q} t) }{P_{kl}(t)}
		$  $\Rightarrow O(M^2)$   
		\STATE $E[n_{ij} | O, T, Q] += p(s(t_{v})=k,s(t_{v+1})=l|O,T,\hat{Q}_{0}) E[n_{ij} | s(0) = k, s(t) = l]$ 
		\ENDFOR
		\ENDFOR
		\STATE 		
		{\footnotesize \emph{Soft}: $O(\hat{M} S^3 + V S^3 M^2 + VS^2 L M^2)$;
		\emph{Hard}: $O(\hat{M} S^3 + V S M^2 + V L M^2)$ }
	\end{algorithmic} 
\end{algorithm}

\subsubsection{Summary of Time Complexity}

To compare the computational cost of different methods, we conducted an asymptotic complexity analysis for the five combinations of \emph{hard} and \emph{soft} EM with the methods \emph{Expm}, \emph{Unif}, and \emph{Eigen} for computing the ESCE. The complexities are summarized in Table~\ref{table:time_complexity}. \emph{Eigen} is the most attractive of the soft methods at $O(VS^3 + VLS^2)$, where $V$ is the number of visits, $S$ is the number of  states, and $L$ is the number of edges.  Its one drawback is that the eigendecomposition may become ill-conditioned at any iteration.  However, in our experiments, with a random initialization, we found Eigen to be successful, and other papers have found similar results \cite{Metzner2007}, although generally with a smaller number of states.  If \emph{Eigen} fails, \emph{Expm} provides an alternative soft method, and \emph{Unif} provides an alternative hard method. \emph{Hard Unif} is often faster than \emph{Expm} in practice, so we recommend running that first to get a sense of how long \emph{Expm} will take, and if it is feasible, run \emph{Expm} afterwards.

\begin{table*}[t]
\small
	\centering	
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	\caption{\small
		Time complexity comparison of all methods in evaluating all required expectations under \emph{Soft/Hard} EM,
		$S$: number of states, $L$: number of edges, $V$: number of visits, $M$: the largest truncation point of the infinite sum for \emph{Unif}, set as $\ulcorner 4 + 6 \sqrt{\hat{q} \hat{t} } + (\hat{q} \hat{t}) \urcorner$, where $\hat{q}= \max_i q_i$, and $\hat{t} = max_{\Delta} \tau_{v}$).
	}
	\begin{tabular}{|l||l|l|l|}
		\hline
		complexity & Expm & Unif & Eigen\\ \hline \hline
		Soft EM & $O(V S^4 + V L S^3)$  & \tabincell{c}{$O(M V^3 + V S^3 M^2$\\$ + V S^2 L M^2)$} & $O(VS^{3}+VLS^{2})$\\ \hline
		Hard EM & $O(V S^4 + V L S^3)$ &		
		\tabincell{c}{     
        $O(M S^3 + V S M^2$ \\  $+V L M^2)$} & N/A\\ \hline		
	\end{tabular}	 
	\label{table:time_complexity}
\end{table*}

%%Table~\ref{table:time_complexity} presents a comparison of the time complexities among the three methods. 
The time complexity comparison between \emph{Expm} and \emph{Unif} depends on the relative size of the state space $S$ and $M$, where $M = \ulcorner 4 + 6 \sqrt{\max_i q_i t } + (\max_i q_i t) \urcorner$ is the largest truncation point of the infinite sum used in \emph{Unif} (see Table~\ref{table:time_complexity}). It follows that \emph{Unif} is more sensitive to $\max_i q_i t$ than \emph{Expm} (quadratic versus log dependency). This is because when \emph{Expm} is evaluated using the scaling and squaring method \cite{Higham2008}, the number of matrix multiplications depends on the number of applications of matrix scaling and squaring, which is $\ulcorner \log_2(||Q t||_1/\theta_{13})\urcorner$, where $\theta_{13}=5.4$ (the \emph{Pade} approximant  with degree 13).  If scaling of $Q$ is required \cite{Higham2008}, then we have $\log_2(||Q t||_1) \leq \log_2(S \max_{i} q_i t)$. Therefore, the running time of \emph{Unif} will vary with $\max q_i  t$ more dramatically than \emph{Expm}. 

%% Like \emph{Eigen}, \emph{Expm} can also fail as noted in previous sections, but is considered more robust overall.
%% The time complexity of \emph{Expm} is less sensitive to $\max_i q_i  t$ than \emph{Unif} method (log versus quadratic dependency). 

When selecting an EM variant, there are three considerations: stability, time, and accuracy. Overall, \emph{soft Eigen} offers the best tradeoff between speed and accuracy. However, if it is not stable, then \emph{soft Expm} will generally have higher accuracy than \emph{hard Unif}, but may be less efficient.

In some applications, event times are distributed irregularly over a discrete timescale.  For example, hospital visits may be identified by their date but not by their time.  In that case, the interval between two events will be a discrete number.  In such cases, events with the same interval, e.g. with five days between visits, can be pooled and the ESCE can be computed once for all such events.  See \cite{LiuNips15} for details, including the supplementary material for complexity analysis.


==> Intro.tex <==



% \section{Outline of Introduction}
% \begin{enumerate}
% \item What is disease progression?  Benefits/goals
% \begin{itemize}
% \item include the optimal decoding as a goal
% \end{itemize}
% The goal of disease progression modeling is to learn a model for the temporal evolution of a disease from sequences of clinical measurements obtained from a longitudinal sample of patients. By distilling population data into a compact representation, disease progression models can yield insights into the disease process through the visualization and analysis of disease trajectories. \textcolor{red}{The models might be used to see the most likely path a disease has taken in terms of stages of the disease, as well as how long it has likely spent in each stage}. In addition, the models can be used to predict the future course of disease in an individual, supporting the development of individualized treatment schedules and improved treatment efficiencies. Furthermore, progression models can support phenotyping by providing a natural similarity measure between trajectories which can be used to group patients based on their progression.

% \item Why hidden variable models?  Use some material from the book chapter

% Hidden variable models are particularly attractive for modeling disease progression for three reasons: 1) they are interpretable and can support the abstraction of a disease state via the latent variables; 2) they can deal with noisy measurements effectively; and 3) any
% prior knowledge or constraints on the temporal evolution of the latent states can be
% captured by a model of the state dynamics. The interpretability of latent state models
% is an attractive feature. Since the latent states have a direct interpretation in the context
% of an experiment, the examination of latent state trajectories (following model
% fitting) is a potentially-powerful tool for gaining insight into complex temporal patterns.
% This is particularly important if the probability distributions obtained from
% latent state modeling are to be used in subsequent analysis steps, such as adjusting
% the tailoring variables in a health intervention.
% \item DT-HMM and its drawbacks

% A standard latent variable model for temporal data is the Hidden Markov Model (HMM). The Discrete Time HMM (DT-HMM) is widely used in speech recognition, robotics, signal processing, and other domains. It assumes that measurement data arrives at a fixed, regular sampling rate, and associates each measurement sample with an instantiated hidden state variable. The DT-HMM is an effective model for a wide range of time series data, such as the outputs of accelerometers, gyroscopes, and photoplethysmographic sensors. However, the fixed sampling rate assumptions that underly the DT-HMM make it an inappropriate model choice for data that is distributed irregularly in time, such as clinical data.

% A further disadvantage of using DT-HMMs to model event data is the fact that transitions in the hidden state are assumed to occur at the sample times. Since event data may be distributed sparsely in time, a more flexible model would allow hidden state transitions to occur between observations. One potential approach to using DT-HMMs with event data would be to set the sampling period fine enough to describe the desired state dynamics and then use a missing data model to address the fact that many sample times will not have an associated measurement. While this approach is frequently-used, it has several undesirable properties. First, the treatment of missing measurements can be both inefficient and inaccurate when the number of observations is sparse relative to the sampling rate. On the other hand, if the discretization is too coarse, many transitions could be collapsed into a single one, obscuring the actual continuous-time dynamics. Second, the sparsity of measurement can itself change over time. For example, during the early stages of a disease visits to a doctor may be infrequent, while in the late stages a patient may need frequent visits to monitor the condition.  The need to tradeoff between the temporal granularity at which state transitions can occur and the number of missing measurements which must be handled is a consequence of using a discrete time model to describe an inherently sparse, continuous-time measurement process.
% \item background on CT-HMM
% \begin{enumerate}
% \item What is CT-HMM?
% \item issues with previous model
% \item include lack of solving optimal decoding as an issue

% A \emph{Continuous-Time} HMM (CT-HMM) is an HMM in which both the transitions between hidden states and the arrival of observations can occur at arbitrary (continuous) times (~\cite{CoxBook1965, JacksonJSS2011}). It is therefore suitable for irregularly-sampled temporal data such as clinical measurements (~\cite{BartolomeoBMC2011,LiuMICCAI2013,Wang2014kdd}). Unfortunately, the additional modeling flexibility provided by CT-HMM comes at the cost of a more complex inference procedure. %during EM-based maximum likelihood parameter learning
% In CT-HMM, not only are the hidden states unobserved, but the \emph{transition times} at which the hidden states are changing are also unobserved. Moreover, multiple unobserved hidden state transitions can occur between two successive observations.  Because of this, not only is expectation maximization (EM) based learning more difficult, but decoding the optimal sequence of state transitions and the expected dwell times, which can be done directly via the Viterbi algorithm in a DT-HMM, also becomes difficult.

% A previous method addressed these challenges by directly maximizing the data likelihood (\cite{JacksonJSS2011}), but this approach is limited to very small model sizes. A general EM framework for continuous-time dynamic Bayesian networks, of which CT-HMM is a special case, was introduced in~\cite{nodelman05}, but that work did not address the question of efficient learning. Consequently, there is a need for efficient CT-HMM learning methods that can scale to large state spaces (e.g. hundreds of states or more)(~\cite{MurilloNIPS2011Complete}), and a method to decode the optimal sequence of state transitions and the expected dwell times.

% \end{enumerate}
% \item Work we build on
% \begin{enumerate}
% \item the work for original CT-HMM paper
% \item the work for fast \textit{Eigen}
% \item the work for optimal decoding
% \end{enumerate}
% \item How we solve
% \begin{enumerate}
% \item solving the CT-HMM learning problem
% \item solving the optimal decoding problem
% \end{enumerate}
% This article describes a computational framework for CT-HMM learning which can efficiently handle a large number of states within an EM framework. It is based on~\cite{LiuNips15}, but includes additional algorithmic details and analysis of the computational cost of model learning. Further, we have improved the complexity of one of
% the approaches by a factor of the number of states, and provided a solution to decoding the optimal state transitions and expected dwell times.  For EM-based learning, we begin in Section~\ref{sec:ctmc} by introducing the mathematical definition of the Continuous-Time Markov Chain (CTMC). In a CTMC, the states are directly observable and there is no measurement process.  For EM-based learning, It turns out that the key computations which are required for CT-HMM learning also arise in fitting CTMC models to data~\cite{Metzner2007,Hobolth2011,TataruBio2011}. Section~\ref{sec:cthmm} describes the addition of a measurement process which extends the CTMC model into a CT-HMM, and introduces the key equations which arise in parameter learning. Multiple approaches to the problem using EM are presented in Section~\ref{sec:em}. These approaches differ in the specific computational methods used in the E-step, and represent different approaches to solving the core computational problem that underlies EM for CT-HMM. In Section~\ref{sec:exp}, we describe the results from an experimental evaluation of CT-HMM using both simulation studies and real-world clinical datasets. 

% For the decoding problem, we decompose the problem into three parts: a) finding the optimal sequence of states at observation times b) finding the optimal sequence of states between observations c) finding the expected dwell times.  For a), we use the variant of the Viterbi algorithm for CT-HMMs that we developed in the EM learning section, for b) we use the method of \cite{Levin2012} and adapt it to the CT-HMM case, and for c) we borrow a transition matrix structure from \cite{Hajiaghayi2014} and combine it with our method for calculating expected dwell times, also developed in the EM learning section.  We visualize several progressions on the Glaucoma dataset.

% These results demonstrate the practical utility of CT-HMM for clinical data modeling. Note that additional updates will be made available through our project website.~\footnote{http://www.computationalhealth.com/projects/ct-hmm-learning} 
% \end{enumerate}

==> RESULTS_EM.tex <==
\subsection{Experimental results}
\label{sec:exp}

We evaluated our EM algorithms in simulation (Sec.~\ref{sec:exp1}) and on two real-world datasets: a glaucoma dataset (Sec.~\ref{sec:exp2}) in which we compare our prediction performance to a state-of-the-art method, and a dataset for Alzheimer's disease (AD, Sec.~\ref{sec:exp3}) where we compare visualized progression trends to recent findings in the literature. Our disease progression models employ 105 (Glaucoma) and 277 (AD) states, representing a significant advance in the ability to work with large models (previous CT-HMM works~\cite{JacksonJSS2011,MurilloNIPS2011Complete,Wang2014kdd} employed fewer than 100 states).  We initialized the rate matrix uniformly with a small random perturbation added to each element. The random perturbation avoids a degenerate configuration for the \emph{Eigen} method, while uniform initialization makes the runtimes comparable across methods. We used balancing for the eigendecomposition. Our timing experiments were run on an early 2015 MacBook Pro Retina with a 3.1 GHz Intel Core i7 processor and 16 GB of memory.

%% In Sec. \ref{sec:exp1}, we test the learning accuracy of all the presented methods on a 5-state complete digraph using synthetic data under different noise levels. In Sec. \ref{sec:exp2}, we apply CT-HMM to model and visualize glaucoma progression using a 2D-grid forwarding model and evaluate its predictive performance on a real glaucoma dataset using a simple procedure to predict continuous future measurements. 
%% %We will show a simple procedure to predict continuous future measurements. 
%% %The prediction performance will be compared to the state-of-the-art method \cite{Medeiros2012} for Glaucoma prediction.
%% In Sec. \ref{sec:exp3}, we demonstrate the use of CT-HMM as an exploratory tool for understanding Alzheimer's disease (AD). A 3D-grid forwarding model is used to capture the dynamic interactions among three selected biomarkers for AD. We will compare the derived state transition trends to the recent findings in AD literatures.

%Our visualization results supports an important recent finding about temporal ordering of amyloid beta level and hippocampus atrophy.

%================
\subsubsection{Simulation on a 5-state Complete Digraph}
\label{sec:exp1}

%with 20 edges 
We test the accuracy of all methods on a 5-state complete digraph with synthetic data generated under different noise levels.
%, which has a directed edge between each state pair. 
%The ground truth $Q$ matrix is set up such that 
Each $q_i$ is randomly drawn from $[1,5]$ and then $q_{ij}$ is drawn from $[0,1]$ and renormalized such that $  \sum_{j \neq i} q_{ij} = q_i$. The state chains are generated from $Q$, such that each chain has a total duration around $T = \frac{100}{\min_i q_i} $, where $\frac{1}{\min_i q_i}$ is the largest mean holding time. The data emission model for state $i$ is set as $N(i, \sigma^2)$, where $\sigma$ varies under different noise level settings.
%with $\sigma = 0.25$.
The observations are then sampled from the state chains with rate $\frac{0.5}{\max_i q_i}$, where $\frac{1}{\max_i q_i}$ is the smallest mean holding time, which should be dense enough to make the chain identifiable. A total of $10^5$ observations are sampled. % sample the chains and observations until the total observation achieves $10^6$.
The average 2-norm relative error 
$\frac{||\hat{q} - q||}{||q||}$ is used as the performance metric, 
where $\hat{q}$ is a vector contains all learned $q_{ij}$ parameters, and  $q$ is the ground truth.

%The simulation results from 5 random runs are listed in Table \ref{table:learn_exp2}, where all methods achieves low error rates. We find that all \textit{Soft} methods achieve significantly better accuracy than \textit{Hard} methods, suggesting that doing soft is superior to doing hard. The three expectation evaluation methods all have good and similar accuracy, which corroborates the findings from \cite{TataruBio2011} for CTMC.

The simulation results from 5 random runs are given in Table~\ref{table:learn_exp2}. \emph{Expm}, \emph{Unif}, and \emph{Eigen} produced nearly identical results, and so they are combined in the table, which focuses on the difference between hard and soft variants. We found \emph{Eigen} to be stable across all runs. All soft methods achieved significantly higher accuracy than hard methods, especially for higher observation noise levels. This can be attributed to the maintenance of the full hidden state distribution, leading to improved robustness to noise.


\begin{table*}[!t]
\small
\centering		
	\caption{ 
	\small	
		The average 2-norm relative error 
		from 5 random runs on a 5-state complete digraph under varying measurement noise levels. 
	}\vskip -0.1in	
	\begin{tabular}{|l||l|l|l|l|l|}
		\hline
		\footnotesize
		Error & $\sigma=1/4$ & $\sigma=3/8$ & $\sigma=1/2$ & $\sigma=1$ & $\sigma=2$ \\ \hline \hline
		Soft & 0.026$\pm$0.008 &  0.032$\pm$0.008 &  0.042$\pm$0.012 & 0.199$\pm$0.084 & 0.510$\pm$0.104 \\ \hline
		Hard & 0.031$\pm$0.009 &  0.197$\pm$0.062 &  0.476$\pm$0.100 & 0.857$\pm$0.080 & 0.925$\pm$0.030 \\ \hline			
	\end{tabular}
	\label{table:learn_exp2}
\end{table*}

\begin{figure}[tb]
	\vskip -0.1in
	\centering
	%\includegraphics[width=0.8\linewidth]{CTHMM_predict_continuous_value.eps}
	\includegraphics[width=14cm]{CTHMM_predict_3subfig.eps}
	\vskip -0.05in
	\caption{	\small
		(a) The 2D-grid state structure for glaucoma progression modeling. (b) Illustration of the prediction of future states from $s(0)=i$.
		(c) One fold of convergence behavior of \textit{Soft(Expm)} on the glaucoma dataset.
	}
	\label{fig:glaucoma}
	\vskip -0.15in
\end{figure}

In the next set of experiments, we used the CT-HMM to analyze and visualize disease progression patterns from two real-world datasets of glaucoma and Alzheimer's Disease (AD), and show predictive performance on the Glaucoma dataset. Both are examples of degenerative disorders where the time course of the disease plays an important role in its etiology and treatment. We demonstrate that CT-HMM can yield insight into disease progression, and we compare the timing results for learning across our family of methods.

\subsubsection{Application of CT-HMM to Predicting Glaucoma Progression}
\label{sec:exp2}

We now describe a 2D CT-HMM for glaucoma progression. Glaucoma is a leading cause of blindness and visual morbidity worldwide \cite{KingmanWHO2004}. This disease is characterized by a slowly progressing optic neuropathy with associated irreversible structural and functional damage. We use a 2D-grid state space model defined by successive value bands of the two main glaucoma markers, Visual Field Index (VFI) (functional marker) and average RNFL (Retinal Nerve Fiber Layer) thickness (structural marker) with forwarding edges (see Fig. \ref{fig:glaucoma-alzheimers}(a)).

Our glaucoma dataset contains 101 glaucomatous eyes from 74 patients followed for an average of 11.7$\pm$4.5 years, and each eye has at least 5 visits (average 7.1$\pm$3.1 visits). There were 63 distinct time intervals. The state space is created so that most states have at least 5 raw measurements mapped to them. All states that are in a direct path between two successive measurements are instantiated, resulting in 105 states.%\footnote{The grid $[100.5~99.5~98~96~93~90~85 ~80:(-10):20]$ is used for Visual Field Index (the functional marker), and the grid $[130:(-5):80 ~70:(-10):30]$ is used for the Retinal Nerve Fiber Layer thickness (the structural marker) for the glaucoma prediction task.} The data emission model is set as a normal distribution with $\mu$ set to the center of the data band, and $\sigma$ set to 0.25 of the band width. 
%Ten-fold cross validation was used with \emph{soft Expm} as the computational approach. Testing proceeded by decoding the first 4 visits using the learned CT-HMM model and then predicting future states and observations.

To predict future continuous measurements, we follow a simple procedure illustrated in Fig.~\ref{fig:glaucoma}(b). Given a testing patient, Viterbi decoding is used to decode the best hidden state path for the past visits. Then, given a future time $t$, the most probable future state is predicted by $j = \max_j P_{ij}(t)$ (blue node), where $i$ is the current state (black node). To predict the continuous measurements, %for each disease marker separately, 
we search for the future time $t_1$ and $t_2$ in a desired resolution when the patient enters and leaves a state having same value range as state $j$ for each disease marker separately.
%, respectively.
%state $j$, respectively. 
%Both $t_1$ and $t_2$ can be found in a desired time resolution by binary searching. 
The measurement at time $t$ can then be computed by linear interpolation between $t_1$ and $t_2$ and the two data bounds of state $j$ for the specified marker ($[b1,b2]$ in Fig. \ref{fig:glaucoma}(b)). 
The mean absolute error (MAE) between the predicted values and the actual measurements was used for performance assessment. The performance of CT-HMM was compared to both conventional linear regression and Bayesian joint linear regression~\cite{Medeiros2012}. 
%For linear regression, the individualized slope was computed from the first 4 prior visits, while 
For the Bayesian method, 
%the best individualized intercepts and slopes were derived using both information from the past visits and 
the joint prior distribution of the four parameters (two intercepts and two slopes) computed from the training set \cite{Medeiros2012} is used alongside the data likelihood. The results in Table~\ref{table:predict} demonstrate the significantly improved performance of CT-HMM.

In Fig.~\ref{fig:glaucoma-alzheimers}(a), we visualize the model trained using the entire glaucoma dataset. Several dominant paths can be identified: there is an early stage containing RNFL thinning with intact vision (blue vertical path in the first column). At RNFL range $[80,85]$, the transition trend reverses and VFI changes become more evident (blue horizontal paths). This $L$ shape in the disease progression supports the finding in~\cite{Wollstein2012} that RNFL thickness of around $77$ microns is a tipping point at which functional deterioration becomes clinically observable with structural deterioration. Our 2D CT-HMM model reveals the non-linear relationship between structural and functional degeneration, yielding insights into the progression process.


\vskip -0.12in
\begin{table*}[htb]
\small
	\centering	
	\caption{ \small
		The mean absolute error (MAE) of predicting the two glaucoma measures.
		($*$ represents that CT-HMM performs significantly better than the competing method under \textit{student t-test}).
	}
	\vskip -0.1in
	\begin{tabular}{|c||c|c|c|}
		\hline
		MAE & CT-HMM  & Bayesian Joint Linear Regression & Linear Regression \\ \hline \hline
		VFI & 4.64 $\pm$ 10.06 & 5.57 $\pm$ 11.11 * ($p=0.005$)
		&  7.00 $\pm$ 12.22  *($p \approx 0.000$) \\ \hline
		RNFL & 7.05 $\pm$ 6.57 &  9.65 $\pm$ 8.42 * ($p \approx 0.000$)
		&  18.13 $\pm$ 20.70 * ($p \approx 0.000$) \\ \hline
	\end{tabular}
	\label{table:predict}
% 	\vskip -0.20in
\end{table*}

%=============

\subsubsection{Application of CT-HMM to Exploratory Analysis of Alzheimer's Disease}

\label{sec:exp3}
We now demonstrate the use of CT-HMM as an exploratory tool to visualize the temporal interaction of disease markers of Alzheimer's Disease (AD). AD is an irreversible neuro-degenerative disease that results in a loss of mental function due to the degeneration of brain tissues. An estimated 5.3 million Americans have AD, yet no prevention or cures have been found~\cite{ADNIweb}. It could be beneficial to visualize the relationship between clinical, imaging, and biochemical markers 
as the pathology evolves, in order to better understand AD progression and develop treatments.

In this experiment, we analyzed the temporal interaction among the three kinds of markers: amyloid beta ($A\beta$) level in cerebral spinal fluid (CSF) (a bio-chemical marker), hippocampus volume (a structural marker), and ADAS cognition score (a functional marker). We obtained the \emph{ADNI} (The \emph{Alzheimer's Disease Neuroimaging Initiative}) dataset from~\cite{ADNIweb}.\footnote{Data were obtained from the ADNI database (\url{adni.loni.usc.edu}). 
	The ADNI was launched in
	2003 as a public-private partnership, led by Principal Investigator Michael W. Weiner,
	MD. The primary goal of ADNI has been to test whether serial magnetic resonance imaging
	(MRI), positron emission tomography (PET), other biological markers, and clinical and
	neuropsychological assessment can be combined to measure the progression of mild
	cognitive impairment (MCI) and early Alzheimerâs disease (AD). For up-to-date information,
	see \url{http://www.adni-info.org}
	}
Our sample included patients with mild cognitive impairment (MCI) and AD who had at least two visits with all three markers present, yielding 206 subjects with an average of $2.38 \pm 0.66$ visits traced in $1.56 \pm 0.86$ years. The dataset contained 3 distinct time intervals at one month resolution. A 3D gridded state space consisting of 277 states with forwarding links was defined such that for each marker, there were 14 bands that spanned its value range. The procedure for constructing the state space and the definition of the data emission model is the same as in the glaucoma experiment. Following CT-HMM learning, the resulting visualization of Alzheimer's disease in Fig.~\ref{fig:glaucoma-alzheimers}(b) supports recent findings that a decrease in the A level of CSF (blue lines) is an early
marker that precedes detectable hippocampus atrophy (green lines) in cognition-normal elderly~\cite{Anne2009}. The CT-HMM disease model and its associated visualization can be used as an exploratory tool to gain insights into health dynamics and generate hypotheses for further investigation by biomedical researchers.

Fig.~\ref{fig:bar-chart-all} gives the average runtime comparison for a single EM iteration between \emph{soft Expm}, \emph{soft Eigen}, and \emph{hard Unif} for both datasets.  \emph{Soft Eigen} with our improvements is 26 times faster than \emph{soft Expm} for the glaucoma experiment, and 35 times faster for the AD experiment.  \emph{Hard Unif} is slightly slower than \emph{soft Eigen}.  We did not include \emph{soft Unif} due to its poor complexity or \emph{hard Eigen} due to its minimal computational benefit in comparison to \emph{soft Eigen}.


\begin{figure}[h]
	\centering
	\ifx\includegraphics[height=3cm]{2D_glaucoma_model_struct.pdf}\hfill\fi
	\includegraphics[height=5.7cm]{two_disease_progress-eps-converted-to.pdf}
	\vskip -0.05in
	\caption{Visualization scheme: (a) Nodes represent states of glaucoma, with the node color encoding the average sojourn time (red to green: 0 to 5 years and above). The blue links between nodes indicate the most probable (i.e. strongest) transitions between adjacent states, selected from among the three allowed transitions (i.e., down, to the right, and diagonally). The line width and the node size reflect the expected count of patients passing through a transition or state. (b) The representation for AD is similar to (a) with the strongest transition from each state being coded as follows: $A\beta$ direction
(blue), hippo (green), cog (red), $A\beta$+hippo (cyan), $A\beta$+cog (magenta), hippo+cog (yellow), $A\beta$+hippo+ cog(black). The node color represents the average sojourn time (red to green: 0 to 3 years and above).}
    %(a) Result of fitting CT-HMM to glaucoma corpus and visualizing state transition probabilities. (b) Alzheimer's disease visualization}
	\label{fig:glaucoma-alzheimers}
\end{figure}
\begin{figure}[h]
	\centering
	\includegraphics[width=10cm]{bar-chart-all-eps-converted-to.pdf}
	\vskip -0.05in
	\caption{Time comparison for the average time per iteration between \emph{soft Expm}, \emph{soft Eigen} and \emph{hard Unif} for both experiments.  \emph{Soft Eigen} is the fastest method, over an order of magnitude faster than \emph{soft Expm} in both cases.  Thus, it should be used unless the eigendecomposition fails, in which case there is a tradeoff between \emph{soft Expm} for accuracy and \emph{hard Unif} for speed.\small%This is the average time to complete a single iteration of EM.  In \emph{Expm}, most of the time is spent computing end-state conditioned expectations.  
		}
	\label{fig:bar-chart-all}
\end{figure}

